An Incrementally Expanding Approach for Updating PageRank on Dynamic Graphs

PageRank is a popular centrality metric that assigns importance to the vertices of a graph based on its neighbors and their score. Efficient parallel algorithms for updating PageRank on dynamic graphs is crucial for various applications, especially as dataset sizes have reached substantial scales. This technical report presents our Dynamic Frontier approach. Given a batch update of edge deletion and insertions, it progressively identifies affected vertices that are likely to change their ranks with minimal overhead. On a server equipped with a 64-core AMD EPYC-7742 processor, our Dynamic Frontier PageRank outperforms Static, Naive-dynamic, and Dynamic Traversal PageRank by 7.8x, 2.9x, and 3.9x respectively - on uniformly random batch updates of size 10^-7 |E| to 10^-3 |E|. In addition, our approach improves performance at an average rate of 1.8x for every doubling of threads.

==> src/alg-naive.tex <==
\begin{algorithm}[!hbt]
\caption{Parallel Naive-dynamic PageRank.}
\label{alg:prnd}
\begin{algorithmic}[1]

\Statex

\Function{$\text{ND}_{\text{WBPR}}$}{$G^t, R^{t-1}$}
  \State $R_{new} \gets R \gets R^{t-1}$
  \ForAll{$i \in [0 .. MAX\_ITERATIONS)$}
    \ForAll{$v \in V^t$ \textbf{in parallel}}
      \State $r \gets (1 - \alpha)/|V^t|$
      \ForAll{$u \in G^t.in(v)$}
        \State $r \gets r + \alpha * R[u] / |G^t.out(u)|$
      \EndFor
      \State $\Delta r \gets |r - R[v]|$ \textbf{;} $R_{new}[v] \gets r$
    \EndFor
    \State \textbf{wait for all threads} (implicit barrier)
    \State $\Delta R \gets l_\infty Norm(R, R_{new})$ \textbf{in parallel}
    \State $swap(R_{new}, R)$
    \State $\rhd$ Ranks converged?
    \If{$\Delta R \le \tau$} \textbf{break}
    \EndIf
  \EndFor
  \Return{$R$}
\EndFunction
\end{algorithmic}
\end{algorithm}




%% Requires (parameters):
% G(V, E): a directed unweighted graph
% R: initial ranks (1/N for static)

%% Parameter values:
% MAX\_ITERATIONS = 500
% DAMPING\_FACTOR = 0.85
% TOLERANCE = 10^-10


==> src/alg-static.tex <==
\begin{algorithm}[!hbt]
\caption{Parallel Static PageRank.}
\label{alg:prst}
\begin{algorithmic}[1]

\Statex

\Function{$\text{Static}_{\text{WBPR}}$}{$G^t$}
  \State $R_{new} \gets R \gets \{1/|V^t|\}$
  \ForAll{$i \in [0 .. MAX\_ITERATIONS)$}
    \ForAll{$v \in V^t$ \textbf{in parallel}}
      \State $r \gets (1 - \alpha)/|V^t|$
      \ForAll{$u \in G^t.in(v)$}
        \State $r \gets r + \alpha * R[u] / |G^t.out(u)|$
      \EndFor
      \State $\Delta r \gets |r - R[v]|$ \textbf{;} $R_{new}[v] \gets r$
    \EndFor
    \State \textbf{wait for all threads} (implicit barrier)
    \State $\Delta R \gets l_\infty Norm(R, R_{new})$ \textbf{in parallel}
    \State $swap(R_{new}, R)$
    \State $\rhd$ Ranks converged?
    \If{$\Delta R \le \tau$} \textbf{break}
    \EndIf
  \EndFor
  \Return{$R$}
\EndFunction
\end{algorithmic}
\end{algorithm}




%% Requires (parameters):
% G(V, E): a directed unweighted graph
% R: initial ranks (1/N for static)

%% Parameter values:
% MAX\_ITERATIONS = 500
% DAMPING\_FACTOR = 0.85
% TOLERANCE = 10^-10


==> src/alg-traversal.tex <==
\begin{algorithm}[!hbt]
\caption{Parallel Dynamic Traversal PageRank.}
\label{alg:prdt}
\begin{algorithmic}[1]
\Require{$\Delta^{t-}, \Delta^{t+}$: Edge deletions and insertions}
\Ensure{$V_A$: Is vertex affected due to current batch update?}

\Statex

\Function{$\text{DT}_{\text{WBPR}}$}{$G^{t-1}, R^{t-1}, \Delta^{t-}, \Delta^{t+}$}
  \State $V_A \gets \{0\}$ \textbf{;} $R_{new} \gets R \gets R^{t-1}$
  \State $\rhd$ Mark initial affected
  \ForAll{$(u, v) \in \Delta^{t-} \cup \Delta^{t+} \textbf{in parallel}$}
    \ForAll{$v' \in G^{t-1}.out(u) \cup G^t.out(u)$}
      \State $visitDfs(V_A, G^t, v')$
    \EndFor
  \EndFor
  \State \textbf{wait for all threads} (implicit barrier)
  \ForAll{$i \in [0 .. MAX\_ITERATIONS)$}
    \ForAll{$v \in V^t$ \textbf{in dynamic parallel}}
      \State $\rhd$ Is vertex not affected?
      \If{$V_A[v] = 0$} \textbf{continue}
      \EndIf
      \State $r \gets (1 - \alpha)/|V^t|$
      \ForAll{$u \in G^t.in(v)$}
        \State $r \gets r + \alpha * R[u] / |G^t.out(u)|$
      \EndFor
      \State $\Delta r \gets |r - R[v]|$ \textbf{;} $R_{new}[v] \gets r$
    \EndFor
    \State \textbf{wait for all threads} (implicit barrier)
    \State $\Delta R \gets l_\infty Norm(R, R_{new})$ \textbf{in parallel}
    \State $swap(R_{new}, R)$
    \State $\rhd$ Ranks converged?
    \If{$\Delta R \le \tau$} \textbf{break}
    \EndIf
  \EndFor
  \Return{$R$}
\EndFunction
\end{algorithmic}
\end{algorithm}




%% Requires (parameters):
% G(V, E): a directed unweighted graph
% R: initial ranks (1/N for static)

%% Parameter values:
% MAX\_ITERATIONS = 500
% DAMPING\_FACTOR = 0.85
% TOLERANCE = 10^-10

